Focusing at a point with caustic crossing for a class of nonlinear equations

We consider the asymptotic behavior of solutions to nonlinear partial differential equations in the limit of short wavelength. For initial data which cause focusing at one point, we highlight critical indexes as far as the influence of the nonlinearity in the neighborhood of the caustic is concerned. Our results generalize some previous ones proved by the first author in the case of nonlinear Schrodinger equations. We apply them to Hartree, Klein-Gordon and wave equations.

==> comments.tex <==
\section{Remarks and comments}
\label{sec:comments}
 
To end this paper, we outline the limits of our results. Nevertheless,
we believe they are an interesting generalization, and provide a
better understanding, of the results of
\cite{Ca2} and \cite{CR2}. 

\subsection{Geometry}First, the geometrical background is very simple;
we consider a 
caustic reduced to a point. This is at least a step in the
understanding of nonlinear phenomena at a caustic in geometrical
optics. More general geometries are considered in \cite{JMRMemoir},
but nonlinear phenomena at the caustic are well understood only
in the case of dissipative equations, leading to absorption of
oscillations.  We emphasized critical indexes in the case of a linear
geometric optics r\'egime, with a focal point, and gave a description
of the critical case. Understanding what may happen in the
supercritical case ($\delta <\alpha (p-1)$ in \eqref{eq:nl4}) should
lead to interesting phenomena. 

\subsection{Other focal points}We consider initial data that focus
at the origin at time $t=1$ (see 
Section~\ref{sec:eps}). It is easy to modify our approach so that
focusing occurs at $(t,x)=(t^\e_j,x^\e_j)$ for any prescribed
$(t^\e_j,x^\e_j)$. The question to know what happens when a
superposition of such initial data (taking different pairs
$(t^\e_j,x^\e_j)$) is natural. Answers are available in the cases of
the critical wave equation \eqref{nlwcrit} and of the semiclassical
nonlinear Schr\"odinger equation \eqref{eq:indiana}, given in
\cite{BG3} and \cite{CFG} (see also \cite{CFGX02})
respectively. In these papers, nonlinear
superposition principles are established. Essentially, the
nonlinearity is negligible when no focusing occurs, for the r\'egimes
considered of those of \emph{linear} geometric optics. When focusing
occurs, it does at a scale which is so small ($\e$ in the case of
\eqref{eq:indiana}) that if the pairs $(t^\e_j,x^\e_j)$ are chosen
``orthogonal'' in a suitable sense, then no interaction occurs. 

\subsection{The role of $\e$} We consider only one small parameter
$\e>0$, as is usual in geometrical optics. However, other small
parameters might play a similar role. As we already mentioned, no
specific scale appears in the study of bounded energy sequences
solutions to the critical wave equation \eqref{nlwcrit}. Indeed,
H.~Bahouri and P.~G\'erard show that several small parameters, of
different orders, are necessary to describe such solutions. This is
because of the scaling of the nonlinearity, which is critical for the
wave equation. 

\subsection{More general initial data} The role of such initial data
as those we consider in \eqref{eq:nl3} or \eqref{eq:nl3bis} could be
better understood. Our argument is that these data cause focusing at
one point, which is the most degenerate caustic. Therefore, the
amplitude growth is the most important predicted by geometrical
optics. Intuitively, this suggests that such data are the only ones,
which are of the same order in the norm $\|\cdot \|_{X,\e}$ (that is,
of order $O(1)$), that make
the nonlinear relevant in \eqref{eq:nl3} or \eqref{eq:nl3bis}. This
means that solutions to Equation~\eqref{eq:nl3} whose initial data are
bounded in the norm $\|\cdot \|_{X,\e}$ are not linearizable if and
only if the initial data can be written as a superposition of such
terms as those we consider, plus a term which generates a linearizable
solution. This vague statement is made rigorous in the cases of
the critical wave equation \eqref{nlwcrit} and of the semiclassical
nonlinear Schr\"odinger equation \eqref{eq:indiana}, in
\cite{BG3} and \cite{CFG} respectively. The proofs of these results
rely on estimates which use finer properties of
Equations~\eqref{eq:lin} and \eqref{eq:nl} than those we state in
Assumptions~\ref{hyp:lin}, \ref{hyp:W-} and \ref{hyp:S}.  The
generality of these results still has to be understood. 

\subsection{Stability properties} In \eqref{eq:nl3}, we
can perturb the initial datum by a term $r^\e$ without changing the
asymptotics of $u^\e$ provided that $\Vert r^\e \Vert_{X,\e}\to 0$ as
$\e \to 0$. This is a stability property for \eqref{eq:nl3}. As we saw
in the proof of Theorem~\ref{theo:critique}, this stability property
stems from a continuity property of the wave operators for \eqref{eq:nl}
(Assumption~\ref{hyp:W-}), and from the global well-posedness for
\eqref{eq:nl} (Assumption~\ref{hyp:S}). 

